Hardening with Scapolite: a DevOps-based Approach for Improved Authoring and Testing of Security-Configuration Guides in Large-Scale Organizations

Security Hardening is the process of configuring IT systems to ensure the security of the systems' components and data they process or store. In many cases, so-called security-configuration guides are used as a basis for security hardening. These guides describe secure configuration settings for components such as operating systems and standard applications. Rigorous testing of security-configuration guides and automated mechanisms for their implementation and validation are necessary since erroneous implementations or checks of hardening guides may severely impact systems' security and functionality. At Siemens, centrally maintained security-configuration guides carry machine-readable information specifying both the implementation and validation of each required configuration step. The guides are maintained within git repositories; automated pipelines generate the artifacts for implementation and checking, e.g., PowerShell scripts for Windows, and carry out testing of these artifacts on AWS images. This paper describes our experiences with our DevOps-inspired approach for authoring, maintaining, and testing security-configuration guides. We want to share these experiences to help other organizations with their security hardening and, thus, increase their systems' security.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> txt/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Every organization or company uses configurable third-party software like operating systems, web servers, email clients et cetera.
The creators of this software choose default configurations tailored towards the functionality and useability of the software.
In some cases, we want a more secure configuration of the software to reduce the attack surface.
Otherwise, attackers can exploit undetected errors, i.e., settings with an insecure value.
Thus, we need to identify the security-relevant configuration settings of the used software, identify the secure value or a set of secure values for each setting, and ensure that each instance of the software used within our company uses a secure value in every relevant setting.
This process is called configuration hardening and is part of the general security hardening of an organization's infrastructure.
We have to monitor our infrastructure's security requirements continuously and configure the systems accordingly.
Therefore, organizations should see their security hardening as a continuous process rather than as a one-time-only task.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{images/old_sec_hardening_proc.pdf}
\caption{The typical process of security hardening.
Dotted lines denote manual tasks.
Every arrow within the box is a task the administrators execute to harden the system.}
\label{fig:hardeningProcess}
\end{figure}

\begin{figure*}[t]
\includegraphics[width=2\columnwidth]{images/new_sec_hardening_proc.pdf}
\caption{Improved process of security hardening}
\label{fig:newHardeningProcess}
\end{figure*}


In the state-of-the-art process of configuration hardening, many manual steps make it prone to such errors.
Figure \ref{fig:hardeningProcess} shows this state-of-the-art configuration hardening process.
There are publicly available security-configuration guides (also called benchmarks, guidelines, or baselines) for various software components, e.g., operating systems like Windows 10, web servers like NGINX, email clients like Outlook, published, e.g., by the CIS\footnote{Center for Internet Security} or the DISA\footnote{Defense Information Systems Agency}.
These guides consist of rules and each rule states which values  should be used for a given setting and why.
One problem is that we cannot use these standard guides without adjustments.
Thus, we have to add settings, remove settings, change values, or create separate profiles.
These adjusted guides then fit the needs of our infrastructure.
Organizations handle configuration hardening nowadays with simple shell scripts like PowerShell or Infrastructure as Code (IaC) approaches like Ansible or Chef.
Therefore, the administrators translate the information about settings and values from the adjusted guide into scripts to apply them.
To verify that the configuration hardening was successful, the administrators use standardized security configuration checks in the OVAL format, vulnerability scanners like Nessus, or custom scripts, e.g., based on PowerShell.
Again, they translate the guides' information into checks.
We need different application scripts because first, the various software to secure need specific application scripts, e.g., rule application on Windows might need PowerShell;
in contrast, rule application on Linux could use Ansible.
Second, there are different use cases, e.g., one administrator cannot use Ansible, so that she would use simple shell scripts instead.
Also, we must support different check types for the check scripts, sometimes even multiple check types for one guide.
The implementation and check authoring are manual tasks.
In Figure~\ref{fig:hardeningProcess}, we did not include the implementation in the input tier because the publishers focus mainly on the check and the documentation aspect;
they do not provide corresponding implementation scripts for all their guides.
In the end, the administrators apply the guides to the systems and verify that every setting has a secure value.
We can detect errors introduced in one of the manual steps only when applying the guides to systems in use, and in many cases, we do not detect them at all.
When the publishers publish a new version of a guide, the administrators must execute the manual steps again.
This repetition of the manual steps increases the risk of introduced errors.

Our solution to this problem of introduced errors is twofold.
First, we present our improved configuration hardening approach that focuses on automation to remove error-prone manual steps.
Second, we present our approach on automatic testing of security-configuration guides to detect errors as soon as possible.

In Figure~\ref{fig:newHardeningProcess}, we depict our improved security hardening process.
We manage all guides in a Markdown-based format called Scapolite.
The tailoring and authoring processes are still manually also in our update hardening process.
The advantage of the Scapolite structure is that we can enrich the guides with automation scripts keeping information about the check, implementation, and documentation together.
The guides now contain all information to automate them as well as all metadata and rationales.
From this single source of truth, we automatically generate scripts to apply the guides to the instances.
At \censor{Siemens}, we use this approach and the corresponding tooling to manage all security-configuration guides, no matter if it is a \censor{Siemens} internal or a CIS guide.
We will later elaborate more on the advantages of our approach to the configuration hardening at \censor{Siemens}, but the most important ones are:
applying the guides takes less time than the manual application;
we can understand the rules better when we keep the information on the application and the metadata together, and we can therefore find errors and inconsistencies more easily;
our tooling supports in every step, and we can reduce the risk of errors significantly.

Nevertheless, our approach and tooling introduce new complexity, and faults in our tooling can lead to new errors.
Therefore, we developed the second part of our solution:
a holistic approach for testing the application and checking of security-configuration guides.
At \censor{Siemens}, we manage all guides with version control systems.
We developed additional tooling to check the guides after every change for potential errors.
We execute this tooling as part of a continuous integration and deployment plan.

If an author changes something in a guide and pushes the changes to our VC server, the pipeline starts.
First, the pipeline automatically generates the scripts based on the information in the guide.
Second, it spawns a new instance of the software as a testbed.
Third, the pipeline executes all phases defined in the test playbook.
This test playbook is a YAML-file in which the author can specify which steps the pipeline should perform to test the security-configuration guide.
Usually, the steps are: 
check the newly spawn instance with generated scripts and verify that the check marks some rules as non-compliant;
The test playbook author specifies the set of compliant rules and the set of non-compliant rules.
There might be an error with a rule or the check scripts' generation if there is a mismatch between this set and the actual set.
Afterward, the pipeline applies all rules to the instance.
If the application script throws an error, there might be an error with the application script's generation.
In the end, the pipeline uses the check script again to verify that the check marks all rules as compliant.
If there are non-compliant rules, this can indicate an error within the application or check script.

Although these are the standard steps of the pipeline, the authors can modify them:
Sometimes, they want to apply all rules but $ X $ rules, because these $X$ rules make the instance inaccessible.
Alternatively, they want to add a check mechanism, e.g., the CIS-CAT tool.
The test playbook language gives the authors the freedom to specify the tests they need for the current guide.

We start a pipeline like this not only once but for every profile in the guide.
We based our tooling on virtualization techniques and use cloud services like AWS to spawn multiple instances in parallel.
Thus, we can give the authors timely direct feedback when their changes cause errors, and we can correlate potential problems directly to their change to ease the debugging.
In summary, our testing approach for security-configuration guides combines multiple existing techniques to find errors in the guides before we apply them to productive systems.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{images/testing_approach.pdf}
\caption{State of the art of security hardening. Dotted lines denote manual tasks.
Every arrow within the box is a task the administrators execute to harden the system.}
\label{fig:oldtestingprocess}
\end{figure}

Our contribution to the field of configuration hardening is twofold:
Our experiences of handling multiple security-configuration guides with multiple profiles modified by various authors within an industrial context might help other organizations improve their configuration hardening process.
We strongly believe that other institutions can significantly improve their infrastructure's security when adapting to a state-of-the-art configuration hardening approach.
Second, we show how we can use existing techniques from the testing and continuous integration domain to reduce the risk of configuration errors in productive systems.
The quality assurance of security-configuration guides does not have to be a manual task.
We hope that our automated testing approach can motivate other researchers and practitioners to create more sophisticated methods to find errors in the guide.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{images/new_testing_approach.pdf}
\caption{State of the art of security hardening. Dotted lines denote manual tasks.
Every arrow within the box is a task the administrators execute to harden the system.}
\label{fig:newtestingprocess}
\end{figure}

==> txt/03_testing_ORIG.tex <==
\section{Our approach to testing}
\label{sec:approach-to-testing}

%- Our approach to security testing
%- - What we want to achieve
%-  - Structure of tests: what to test:
%- - test cases
%- - order of tests
%-    - specification in yaml file which is stored together with baselines sources and contains also expected results
%-  - Best practice in designing tests
%-  - Execution of tests 
%-    - Pipeline integration
%-    - DOCKER IMAGE AS GITLAB RUNNER
%-    - AWS / Virtualbox
%-    - Documentation of test results (logs for inverstigation, overview which can be used for updating test spec)
%-    NAME OF THE FORMAT ?
% Graphical representation of old process of testing


When considering the challenge to support both automated implementation and checking of security-configuration guidelines, then perhaps the moment just after is already a good time to retake into account a famous quote, last time widely used in a superhero, comic movie: “With great power, comes great responsibility”. When one team is responsible for generating, based on machine-readable security-configuration guidelines, a set of hardening scripts capable of improving the security posture of various products and solutions within an enterprise, the force of this team is indeed great. Thus, the responsibility for their work must be at least as great as their force, otherwise the other side of this powerful weapon could cut, especially if a misconfigured security rule is not discovered in time, before running scripts on production systems.

Without prior experience in the Security Configuration Management field, it may be hard to anticipate how challenging it is to have a good quality level for your set of configurations, no matter the format you're using. Actually, the higher your test coverage percentage is, the greater your product's quality will be. Using automated tests in the way described by the CI/CD approach did not reduce at all the effort required for managing security guidelines, but even more so, without this testing manner, the whole test coverage percentage would have remained at low rates. The testing complexity is increased due to the use of numerous variables used when scripts are generated, like: 
\begin{itemize}
    \item OS’s family(Windows, Unix)
    \item OS’s system type(client vs. server) : Windows 10, Windows Server (2016, 2019)
    \item Server role: Domain Controller, Member Server
    \item OS versions: 1809, 1909, 2004 
    \item Specific configuration profile, usually based on risk based classification of enterprise assets
\end{itemize}

At Siemens, for testing a security-configuration guideline written for a server OS system, like Windows Server 2019, one will have a different version-control repository for each different OS version(e.g. 1909, 2004). Based on the content in that repository, one set of scripts will be created for each server role(e.g. Domain Controller, Member server). Within each set of scripts 27 profiles are generated, due to the risk-based asset classification model used at Siemens, which combines three values, representing the Confidentiality, Integrity and Availability levels, each going from 1 to 3.
Therefore, by covering many guidelines, as can be deduced from the above real-life example, the number of the test scenarios will grow massively.

\subsection{What we want to achieve}

Considering the diversity of the scenarios described above, in order to discover at the right time any kind of issues which may introduce security flaws, mostly due to misconfigurations on systems  to be hardened, the only option we had was to find a way to automatically test as many guidelines as possible, every time a change was performed:
\begin{enumerate}
    \item in the scapolite source files of a given guideline, for any of its versions, in order to verify if the impact of that particular change will be indeed the desired one: e.g. an automation associated with a given non-compliant rule was recently improved, therefore one will need to automatically detect if this rule becomes compliant
    \item on the target system, by any reasons: e.g. a new Amazon Machine Image(AMI)  was published for a given version of an OS image; thus, one needs to assess the new results after running the hardening scripts against this particular AMI. If changes are detected, automate as much as possible the investigation process, by identifying at each intermediary test phase, the improvements or the deteriorations relative to last known state. 
\end{enumerate}
Our testing approach has also similar goals as unit testing for an application: we're testing individual parts of our guidelines to ensure each of them behaves as expected and as confirmed by the results identified during last test iteraton, which after some anaylsis, could become the new, updated ground truth.

\subsection{Structure of the test file}

The structure we designed for the test file contains not only guidance on how actual tests will be performed, but also a comprehensive set of expected results, reffered in our approach as \emph{validations}, if we're not anymore in the initial phase of the testing process. One could think that even in the initial phase, the expected results for each testing stage should be known, as they broadly contain the compliance status of every rule currently tested. In our experience, adding validations on an empty test skeleton, as well as updating the ones currently in place were a couple of activities which have to be performed automatically, as this saves us time, removes omissions and is more comfortable.

\begin{listing}[!htb]
\begin{code}
\begin{minted}[fontsize=\footnotesize,firstline=1,linenos,highlightlines={2,4,8-11},breaklines]{md}

os_family: WINDOWS
os_image: WinServer2019
os_image_version: 1909
ciscat_version: v4.0.22
testruns:
- name: WS19 1909 ACP 111 DC ...
- name: WS19 1909 ACP 222 DC ...
- name: WS19 1909 ACP 333 DC
  ps_scripts_relative_path: for_DC
  testrun_siemens_ps_profile: acp333
  activities:
    - id: initial_powershell_check ...
    - id: apply_all ...
    - id: check_after_apply_all_with_ps ...
    - id: revert_all ...
    - id: check_after_revert_with_ps
      type: siemens_ps_scripts
      sub_type: check_all
      blacklist_rules:
      validations:
      - sub_type: compare
        compare_with: initial_powershell_check
        expected:
          rules_passed_only_here: [BL942-0063, BL942-0936, BL942-0981, BL942-3111, BL942-3651, BL942-4046]
          rules_passed_only_there: []
          rules_failed_only_here: []
          rules_failed_only_there: [BL942-0063, BL942-0936, BL942-0981, BL942-3111, BL942-3651, BL942-4046]
          rules_unknown_only_here: []
          rules_unknown_only_there: []
      - sub_type: compare ...          
      - sub_type: count
        expected:
          blacklist_rules: 0
          compliant_checks: 79
          non_compliant_checks: 328
          empty_checks: 46
          unknown_checks: 46
      - sub_type: by_id ...
      - sub_type: by_id
        result: compliant_checks
        check_ids: [BL942-0051, BL942-0063, BL942-0081, BL942-0281, BL942-0421, BL942-0571, BL942-0636, BL942-0931, ... ] 
     - sub_type: by_id
        result: non_compliant_checks
        check_ids: [BL942-0005, BL942-0006_sub_0, BL942-0006_sub_1, BL942-0007, BL942-0020, BL942-0031, BL942-0044, BL942-0050, BL942-0077, BL942-0088, ...]
      - sub_type: by_id ...
      - sub_type: by_id ...  

\end{minted}
\caption{Summarised version of a testfile}
\label{lst:gpo_automation}
\end{code}
\end{listing}


In the above example, which is written in YAML,  one could notice that within a testfile there are some global key-value pairs, identifying the specific OS image this guideline was written for, as well as some versions of the required tools. The testfile contains afterwards \emph{an unordered list of testruns}, each of them specifying a different hardening profile, an list of \emph{ordered list of activities} and, where applicable, the subset of scripts to be used, depending on the server role we want to test. The list of activities specify which exact steps the test should include, in which order they should be executed and, for each activity, its own parameters required for modeling the way this test stage gets executed, as well as \emph{an unordered list of validations}, if they are already known. 

The order of the list of activities is very important, as we want to assess system's overall status in different situations, knowing what happened before on that system. The most common order we used in our tests is: 
\begin{enumerate}
    \item check-rules 
    \item apply-rules
    \item check-rules
    \item revert-rules
    \item check-rules
\end{enumerate}

In the \emph{initial check-rules}, we're expecting to get a status representative for a just deployed instance, before we start to alter its security status with our scripts. In the next stage, called \emph{apply-rules}, we're improving the security posture of the system under test, by applying all the automated implementations in the guideline, not before taking a backup for preserving the initial values. The next phase is the \emph{check-rules after apply}, which assess all the automated rules again, to see which are now compliant, but also we automatically compare the new status the initial one. In order to verify that the hardening scripts are able to set secure configurations back to their initial values, the  \emph{revert-rules} test step is added and, after its execution, the last \emph{check-rules after revert} stage is included, in order to verify the status of the reverted rules, usually performing automatically a comparison with the very initial status.

If requested, validations are parsed, validated and updated at the end of the testrun itself.In  \emph{count validations} we're verifying the number of rules of some kind, like non-compliant, whereas the specific IDs of these rules are verified in \emph{by-id validations}. The \emph{compare validations} are used to perform a comparison between given results, like  non-compliant rules in the after-apply check stage and same type of results in the initial-check stage.

\subsection{Best practices when writing testfiles}

Because it is mandatory to have a solid ground truth, determining the actual status, at any stage, could also be divided into two sub-tasks, where the situation allows for parity between two testing tools: e.g. 
\begin{enumerate}
    \item Initial check with Siemens Powershell scripts
    \item Initial check with CIS-CAT’s Assessor, using the same hardening profile. 
\end{enumerate}
This is useful for double-checking the results of our scripts, by analysing the differences between Siemens checks and CIS’s checks.

 This is also the most common order of activities in a testfile, because we’re checking with various available tools, after and before major changes of system’s security configuration, like the ones brought by apply and revert rules.
 
 By design, this activity in particular has the greatest potential to create issues regarding the management interface used for interacting with the system to be hardened. Therefore, besides other parameters, applying can be done in two different manners: if we already knew the specific rules which could be disruptive for the system under test, we could add them into a list of excepted rules, which will never be applied, if we configure the script execution like that, but all other rules will be applied at once. On the other hand, if we don’t already know all the problematic rules, we could add a parameter that changes the way rules are applied, from all-at-once to one-by-one, in order to detect after which specific rule the automation stops and, in the end, determine the exhaustive list of rules which should be skipped.
 
 Check after apply is the step that determines the overall impact of applying the hardening scripts against a given system, relative to the levels identified by the initial check phase. One could also think that, besides performing an automated double-check at the same step (compare current results identified by our scripts with the ones reported by CIS-CAT Assessor), another useful feature would be to compare also the current results after apply with ones from initial check, in order to confirm that the rules reported as successfully implemented are currently compliant, even if some of them were not in the initial check phase.

Revert rules is, besides the phase where rules are applied, another test step where changes in the security configuration are performed, but does not have, if done correctly, the potential to create so much harm. The purpose of this apparently inoffensive testing phase is to test, for each rule where it’s possible, if the value backed up before applying a given rule was properly stored and apply back, allowing for a safe return to the initial status. 

\subsection{ Management of the YAML test files}

An obvious option for keeping a YAML testfile per each security guideline we are currently managing was to store this input file in the same branch of the VCS project where the scapolite source files were stored.
Also, if our tool is instructed via a parameter to perform an update of the current YAML testfile, based on current results identified, we’ll store both output files in the same artifacts path: last known testfile and its updated version, for which differences  should be analyzed. 
If this new version contains indeed a set of results which should be considered as the new reference, this new file could be considered as the input testfile in the next testing iteration.

Our inspiration of handling the testfile came from the way Gitlab defines the CI behavior of projects stored in their environment, using the 
".gitlab-ci.yml" file created in each project's root directory. Similarly, in the root directory of each security-configuration guideline repository we manage, a testfile called ".scapolite\textunderscore tests.yml" exists and its content is used for performing new tests automatically and for auto-validation of latest results.

\subsection { Execution of tests }

CI/CD principles offered us a good way to integrate and conditionally execute, if requested, this testing stage, because a pipeline was already working for generating scripts based on scapolite source files.

Therefore, the next step would have been to create a new test stage, and configure its jobs to automatically test each new set of scripts generated after every commit. However, we noticed that sometimes a series of small changes will be performed over some hours in the guideline repository, so it would have made absolutely non-sense to let the tests run automatically. So, we conditioned the test execution stage by setting a binary value for a pipeline variable called “EXECUTE\textunderscore TESTS”(default state is False). ) and when this variable is True, the stage is triggered and tests are performed. 

For the testing stage, which we perform right now in AWS's EC2 environment, currently the CI pipeline uses a different Docker image than the other stages, as the testing stage has specific requirements: the container created based on this image has, among other required libraries for our test framework, tools like Ansible and Vagrant configured and ready to use, as well as the "vagrant-aws" and "vagrant-aws-winrm" plugins installed. Each time a new change was made on the framework itself, we rebuild a new Docker image and push it to local registry. However, before running tests in EC2, instead of the docker image, we were using a local server in our datacenter, where Virtualbox was installed. This server was registered as a runner for some CI jobs, depending on their tags. 

The testing framework, to which we will refer as the \emph{Scapolite Workbench}, requires some environment variables (for example, to access AWS resources), some configuration files (for example, to extract the AMI-ID and the credentials for the desired version of the OS image specified in the testfile), as well as various input parameters, two of the ones worthy of being mentioned are the input set of scripts, as well as the test file itself.

\begin{figure}[t]
\includegraphics[width=\columnwidth]{images/aws_workflow.jpg}
\caption{AWS workflow}
\label{fig:hardeningworkflow}
\end{figure}
\ref{fig:hardeningworkflow}


\subsection { Documentation of testresults } 
NOTE: Talk about -  Summary feature.

NOTE: Changing env. Virtualbox limitations vs scalability of aws

==> txt/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> txt/W_related_work.tex <==
\section{Related Work}
\label{sec:relatedwork}

First, we present the current work on configuration management in general and security hardening in particular.
Second, we discuss approaches similar to our testing approach.

In past, reseachers investigated heavily in misconfiguration in general, and security misconfiguration in particular ~\cite{Dietrich:2018:ISO:3243734.3243794,Tang:2015:HCM:2815400.2815401,Continella:2018:THB:3274694.3274736,Jha2017,Xu:2015:SAT:2775083.2791577}.
Dietrich et al. show in their study that security misconfigurations are very common and a severe problem.
According to their data, manual configuration, vague or no process, and poor internal documentation are the main environmental factors that we could solve with a better approach and tooling.

% BG: Ist die related work unten nicht einfach out-of-scope für uns? Darin geht es darum, wie man sichere Konfigurationen findet, bei uns geht es darum, bekannte sichere Konfigurationen zu managen und automatisiert umzusetzen.
% PS: Ich würde die drin lassen, da ich wieder versuchen würde, in die Configuration-management Schiene zu kommen. Ich hoffe, dass ein Author oder Ko-author im Gremium sitzt und sich wegen des Zitats geschmeichelt fühlt ... 
% BG: "security smell" bezieht sich doch auf Fehler im Code und nicht Fehler in der Konfiguration ... insofern verstehe ich nicht, worauf Du Dich beziehst. Sollen die Skripte an sich auf Sicherheitsmängel geprüft werden (was eine völlig neue Baustelle ist, die wir bislang ausser acht gelassen haben) oder das, was die Skripte umsetzen? 
% BG: Vielleicht kann man diese related work besser beschreiben als Dinge, die den Autoren helfen, die richtigen Konfigurationen für die Benchmarks herauszufinden -- wir setzen dann beim nächsten Schritt an, wenn es darum geht, dieses Wissen dann in Benchmarks umzuwandeln?
Many researchers investigated  how we can detect and remove misconfigurations~\cite{Rahman:2019:SSS:3339505.3339528,Santolucito:2017:SCF:3152284.3133888,Keller2008,Su:2007:AIC:1323293.1294284}.
Rahman et al.~\cite{Rahman:2019:SSS:3339505.3339528} analyzed thousands of Infrastructure-as-a-Code (IaaC) scripts to identify insecure configurations.
We use the security guides and generate the guides' scripts to avoid security smells in our use case.
Nevertheless, we could check our generated scripts with their approach as an additional quality gate.
The framework \textit{ConfigV}~\cite{Santolucito:2017:SCF:3152284.3133888} learns good configuration settings based on many given configuration files, but we cannot learn the security settings the same way; we need expert knowledge for that.
% BG: Auch der nächste Punkt gehört zu "Dingen, die man verwenden kann", um sichere Settings zu finden ... ich denke "we cannot use" ist falsch, da es sich um ein Problem handelt, was orthogonal ist .
Similarly, we cannot use SPEX~\cite{Xu:2013:BUM:2517349.2522727} as we do not have the source code of the programs we want to configure, although the vendors of this software could use such an approach to create guides for their software.
%BG Jetzt kommt ein anderes Hauptthema, nämlich Forschung, um die Konfiguration von Systemen einfacher handhabbar zu machen, das könnte man vielleicht vorausstellen...
The Elektra framework~\cite{Raab2020} unifies how we can access configuration settings and creates a central structure for accessing and manipulated configuration settings.
The more software would use concepts likes Elektra, the more we could include these abstract descriptions in our Scapolite files to combine both worlds' best;
for the remaining settings, we would use the scripts described above as a fallback option.
%BG: "Could not use" ist wieder seltsam -- ich würde einfach sagen, dass es ähnlich zu Elektra ist.
Xu et al.~\cite{Xu2016} developed a similar approach to Elektra that we could not use for similar reasons.
Furthermore, they showed~\cite{Xu:2015:HYG:2786805.2786852} convincingly that the configuration's complexity is overwhelming users and systems administrators.
The results of the study underline how important security experts and security guides are in supporting the administrators.
% Da weißt du am besten, wie man den Verweis auf uns selbst verschleiert ... mir kommt das arg komisch vor ... und ich frage mich, ob wir uns nich selbst in der Fussnote weiter oben über den Import externer Baselines zitieren können. 

% Hier sind wir nicht consistent, oben reden wir von ComplianceAsCode, das müssen wir noch auflösen
The ComplianceAsCode~\cite{complianceAsCode,preisler:haicman:UsenixLisa:2017} is very close to the presented approach.
They maintain their security-configuration guides for various Linux systems in a git repository and represent every rule with one file.
This file references other files, e.g., with scripts for automated checking.
Nevertheless, some drawbacks prevented us from using OpenScap.
First, their focus on Linux-based operating systems made it unattractive as it did not support our primary use case of Windows hardening.
%BG: Der zweite Grund gefällt mir nicht ...
%BG: Ich habe vielleicht falsch eingefügt: ich wollte den Format-Satz Zeile 40 und 41 gestrichen haben -- Zeile 43 "Nonetheless" kann bleiben
Second, we could hardly convince our internal authors to write and manage the guides in the ComplianceAsCode format; 
however, they accepted the markdown for documentation and YAML for the structural data approach.
% BG: Nächster Satz: Naja OpenScap ist ja weniger ein Format als ein gesamter Build-Prozess -- den Satz würde ich streichen, insb. da wir ja noch Platz brauchen
%Nonetheless, it would ease the security configuration enormously if the publishers distributed their guides in the OpenScap format so that documentation, check, and implementation are more aligned.

Software testing is a well-researched discipline, and every year, new articles add more information to the general knowledge~\cite{9286051,9286080,9159077,9159091,9159060,9159084,9286071,9286121,9285999,9286104}.
Therefore, we can only refer to a fraction of all available and valuable testing research.
Many researchers, e.g., \cite{9159084,10.1145/3395363.3397365} use sophisticated testing approaches to find security-relevant bugs or leaks in software.
In contrast, we use testing approaches to find bugs in the security-configuration guides, not the software itself.
In the industry, there is a strong need for automated testing, especially in the DevOps scenarios~\cite{9155725}, but also some obstacles to overcome, e.g., when testing a software's graphical user interface~\cite{9155991}.
Since we use our approach productively at \censor{Siemens}, we had to overcome similar problems as the researchers above.
The closest research to our testing of security-configuration guides is the work of Spichkova et al.~\cite{SPICHKOVA20203610} .
Their tool VM2 creates VM images and hardens them automatically with given security-configuration guides.
They also use the CIS's guides, but they see guides as given and immutable, whereas we include in our approach the constant update and maintenance of the guides to adjust them to a company's security policy.
Furthermore, they focus on the combination of Linux-based OSs and Ansible.
In contrast, the diversity of technologies within \censor{Siemens} forced us to support different application and check modes in our approach.

